MotionScript: Natural Language Descriptions for Expressive 3D Human Motions

We introduce MotionScript, a novel framework for generating highly detailed, natural language descriptions of 3D human motions. Unlike existing motion datasets that rely on broad action labels or generic captions, MotionScript provides fine-grained, structured descriptions that capture the full complexity of human movement including expressive actions (e.g., emotions, stylistic walking) and interactions beyond standard motion capture datasets. MotionScript serves as both a descriptive tool and a training resource for text-to-motion models, enabling the synthesis of highly realistic and diverse human motions from text. By augmenting motion datasets with MotionScript captions, we demonstrate significant improvements in out-of-distribution motion generation, allowing large language models (LLMs) to generate motions that extend beyond existing data. Additionally, MotionScript opens new applications in animation, virtual human simulation, and robotics, providing an interpretable bridge between intuitive descriptions and motion synthesis. To the best of our knowledge, this is the first attempt to systematically translate 3D motion into structured natural language without requiring training data.

==> figures_and_tables_tex_files/fig3.tex <==
\begin{figure}[b]
    \centering
    \includegraphics[width=\columnwidth]{figures/timeline_v2.pdf}
    \caption{Timecode: chronological order of \textit{motioncodes}.}
    \label{fig:ChronologicalOrder}
\end{figure}

==> figures_and_tables_tex_files/tab1.tex <==
    \begin{table*}[]
        \footnotesize
        \begin{tabular}{@{}llll@{}}
        Posecode    & Axes and Ordinal Categories                                                             &  &  \\ \cmidrule(r){1-2}
        Orientation & x: lying flat forward,  leaning forward,  slightly leaning forward,  neutral ,  slightly leaning backward,  leaning backward,  lying flat backward                                                                                                                                        &  &  \\
                    & y: leaning left,  slightly leaning left,  slightly leaning right,  neutral,  slightly leaning right,  slightly leaning left,  leaning right                        &  &  \\
                    & z: about-face turned clockwise,  completely turned clockwise,  moderately turned clockwise,  slightly turned clockwise,  neutral,  &  &  \\
                    & slightly turned counter-clockwise, 
                     moderately turned counter-clockwise  completely turned counter-clockwise,  about-face turned counter-clockwise &  &  \\ \cmidrule(r){1-2}
        Translation & x: significant left,  left,  slightly left,   middle,  slightly right,  right,  significant right                                                                                                                                                                                        &  &  \\
                    & y: significant downward,  downward,  slightly downward,  middle, slightly upward,  upward,  significant upward                                                                                                                                                                          &  &  \\
                    & z: significant backward,  backward,  slightly backward,  middle,  slightly forward,  forward,  significant forward                                                                                                                                                                      &  & 
        \end{tabular}
        \caption{Introduced Posecodes. % for managing body rotations and translations Over Time. 
        % \textcolor{red}{This could be in Sup. materials...?}
        }
        
        \label{tab:posecode}
    \end{table*}

==> sections/x_application.tex <==
\clearpage
\setcounter{page}{1}
\maketitlesupplementary


\section{Supplementary}

% In this section we provide more details on how we designed our Motion-Script algorithm and more details on our rules, thresholds, etc in Section \ref{sup_motionscript_algorithm} as well as an ablation study to evaluate the contribution of each component i.e. eligibility, pose-injection, subject detection, intensity adjectives and velocity adjective in Section \ref{sup_motionscript_algorithm}. We provide more results on recent text-to-motion baselines, motion-retrieval, and Motion-to-text (T2M2T) in Section \ref{sup_results_on_recent}. We also include our human-study on generated text from Motion-Script and generated motions from different applications trained on our data in Section \ref{sup_human_study}
% Code is available on GitHub Page. We provide the process of the training and evaluation of the trained models, the pre-trained
% model files, the demo, and example results.


% \subsection{Motionscript Algorithm}
% \label{sup_motionscript_algorithm}

% \subsection{Ablation-Study}
% \label{sup_ablation_study}

% \subsection{Quantitative Evaluation Extended}
% \label{sup_results_on_recent}

% \subsection{Qulitative Results Extended}


% \subsection{Human-Study}
% \label{sup_human_study}



% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=1\linewidth]{figures/sample1_table.png}
%     \caption{Description: His left knee, his right elbow and his right knee are straight and then, his
% right knee is markedly bending and concurrently, the left knee, the right elbow and the
% right knee are unbent and with that alignment, his right elbow is fairly bending. Right
% after, the left elbow is partially bent, then, their left elbow is bending a bit,
% moderately distances from the other one smoothly. Meanwhile, their body is leaning left greatly. In
% the following moment, the right hand is slightly spreading out from the other one at
% a steady rate.  }
%     \label{fig:example2}
% \end{figure}


% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=1\linewidth]{figures/sample2_table.png}
%     \caption{Description: The knees are straight, with that alignment, their right knee bends significantly. Simultaneously, her elbows
% are barely bent and with that alignment, their left elbow is fairly bending, right after,
% it moderately distances from their right elbow with no rush. Concurrently, their right elbow is
% bent a bit, from that stance, the right elbow is barely bending at a normal
% speed and concurrently, the body significantly leans left. The left hand slightly moves away from
% the right hand at a normal speed. }
%     \label{fig:example2}
% \end{figure}



In this supplementary material, we present visualizations of the captions generated by our models, as well as results from models trained using our augmented dataset. Given the limited time available for preparing supplementary materials and the extensive time required for our experiments, we plan to conduct an ablation study, additional experiments, and human-study in preparation for the rebuttal period. 

\subsection{Motion Segmentation Algorithm}

\vspace{-1mm}
\begin{algorithm}
\caption{Motion Segmentation algorithm}
\label{algorithm_motion_detection}
\begin{algorithmic}[1]
\State \textbf{input}:
    \Statex - Posecode Sequence: Numerical values representing pose categories.
    \Statex - Maximum Range: Maximum segment length
\vspace{+1mm}

\Procedure{DetectMotions}{Posecode Sequence, Maximum Range}
    \For{each pose in Posecode Sequence}
        \State Identify changes in \textbf{posecode} categories (positive or negative direction).
        \State Merge adjacent same-direction poses into one motion segment.
        \State Calculate motion attributes i.e. spatial and temproal for each segment.
        \State Store detected motions with their parameters.
    \EndFor
    \State \textbf{return} Detected Motions
\EndProcedure
\end{algorithmic}
\end{algorithm}
\vspace{-4mm}

